In memoriam Leonid V. Keldysh

Leonid Keldysh -- one of the most influential theoretical physicists of the 20th century -- passed away in November 2016. Keldysh is best known for the diagrammatic formulation of real-time (nonequilibrium) Green functions theory and for the theory of strong field ionization of atoms. Both theories profoundly changed large areas of theoretical physics and stimulated important experiments. Both these discoveries emerged almost simultaneously -- like Einstein, also Keldysh had his \textit{annus mirabilis} -- the year 1964. But the list of his theoretical developments is much broader and is briefly reviewed here.

==> Additional_Packages/subfig/README <==
Manifest and Documentation for the `subfig' package (version 1.3).
------------------------------------------------------------------------

This directory contains version 1.3 of the subfig package.  In a UNIX
or UNIX-like command shell, use `make' to extract the subfig package
and run the local tests.


MANIFEST:
---------
  The following files as well as the derivative files `subfig.sty' and
  `altsf.cfg' constitute the subfig package and are considered as "the
  work" under the LaTeX Project Public License (LPPL 1.3 or later).

Makefile           UNIX makefile to extract the subfig package
                       and related material.
README             This file.
subfig.dtx         The documented subfig package.
subfig.ins         The subfig package installation file.
subfig.pdf         The subfig package documentation (in PDF).
test1.tex          Test one: Basic checks and examples.
test2.tex          Test two: Check for extra space around figure
test3.tex          Test four: Test of optional args and \subref.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test of continued figures.
test6.tex          Test six: Test of options and option interaction.
test7.tex          Test seven: Test of class/package misuse of \let.


FILES AFTER `make':
-------------------
Makefile           UNIX makefile to extract the subfig package
                       and related material.
README             This file.
altsf.cfg          A subfig configuration file (which make the subfig 
                        package act similar to the subfigure package).
ltxdoc.cfg         Configuration file to print change history and
                       index on the subfig package documentation.       
subfig.dtx         The documented subfig package.
subfig.ins         The subfig package installation file.
subfig.pdf         The subfig package documentation (in PDF).
subfig.ps          The subfig package documentation (in PostScript).
subfig.sty         The subfig package 
test1.ps           Results of test one.
test1.tex          Test one: Basic checks and examples.
test2.ps           Results of test two.
test2.tex          Test two: Check for extra space around figure
test3.ps           Results of test three.
test3.tex          Test four: Test of optional args and \subref.
test4.pdf          Results of test four.
test4.tex          Test four: Test of interaction with hyperref.
test5.ps           Results of test five.
test5.tex          Test five: Test of continued figures.
test6.ps           Results of test six.
test6.tex          Test six: Test of options and option interaction.
test7.tex          Test seven: Test of class/package misuse of \let.
test7a.ps          Log from test seven run.
test7b.ps          Results of test seven.


NOTES:
------

1. To verify the results of the test(s) (which are run using the
   preferred options), compare with the test(s) found at:
   http://www.cs.cmu.edu/~sdc/latex/subfig.13/

2. This version of the subfig package removes a "feature" which
   allowed a line break to occur between two subfloats separated
   by whitespace instead of requiring an explicit "\\".  If this
   "feature" was used to position sub-floats, they may now be
   incorrectly displayed.

   If this occurs, the solution is to add an expicit linebreak
   between the problem sub-floats.  For example, the following
   to the left would seem to work correctly, but suppressed
   the "farskip" placing the figures too close together and 
   will, now, no longer work.  It should be written as on the
   left.

   \begin{figure}                  \begin{figure}		
     \centering	                     \centering		
       \subfloat[One.]{...}%	       \subfloat[One.]{...}	
     \hspace{.25in}%		     \hspace{.25in}%		
       \subfloat[Two.]{...}	       \subfloat[Two.]{...} \\	
       \subfloat[Three.]{...}%         \subfloat[Three.]{...}	
     \hspace{.25in}%		     \hspace{.25in}%		
       \subfloat[Four.]{...}%	       \subfloat[Four.]{...}	
     \caption{Simple Case.}	     \caption{Simple Case.}	
   \end{figure}                    \end{figure}               










